Understanding BLOOM: An empirical study on diverse NLP tasks

We view the landscape of large language models (LLMs) through the lens of the recently released BLOOM model to understand the performance of BLOOM and other decoder-only LLMs compared to BERT-style encoder-only models. We achieve this by evaluating the smaller BLOOM model variants (\textit{350m/560m} and \textit{1b3/1b7}) on several NLP benchmark datasets and popular leaderboards. We make the following observations: (1) BLOOM performance does not scale with parameter size, unlike other LLMs like GPT and BERT. Experiments fine-tuning BLOOM models show that the 560m variant performs similarly to or better than the 1b7 variant, (2) Zero-shot cross-lingual and multi-lingual fine-tuning experiments show that BLOOM is at par or worse than monolingual GPT-2 models, and (3) Toxicity analysis of prompt-based text generation using the RealToxicityPrompts dataset shows that the text generated by BLOOM is at least 17\% less toxic than GPT-2 and GPT-3 models.

==> other_material.tex <==

% These instructions are for authors submitting papers to ACL 2023 using \LaTeX. They are not self-contained. All authors must follow the general instructions for *ACL proceedings,\footnote{\url{http://acl-org.github.io/ACLPUB/formatting.html}} as well as guidelines set forth in the ACL 2023 call for papers.\footnote{\url{https://2023.aclweb.org/calls/main_conference/}} This document contains additional instructions for the \LaTeX{} style files.
% The templates include the \LaTeX{} source of this document (\texttt{acl2023.tex}),
% the \LaTeX{} style file used to format it (\texttt{acl2023.sty}),
% an ACL bibliography style (\texttt{acl\_natbib.bst}),
% an example bibliography (\texttt{custom.bib}),
% and the bibliography for the ACL Anthology (\texttt{anthology.bib}).



\iffalse
Start with LLMs

few shot learning with LLMs


investigate bloom
- what hypotheses are we exploring in investigating bloom?
- what is our means to this end?
criteria - tasks, explainability, multi-lingual, linguistic features (probing), how to use (possible)
\fi 

%\textit{(insert a couple of sentences on large language models)}

 %including GLUE-language understanding, prompt-based zero-shot and few-shot text classification and extraction, question answering, prompt-based text generation, named entity recognition, and multi-lingual text classification to understand model strengths/weaknesses and behavior. 
%there exist other variants of the BLOOM model with fewer parameters\footnote{\url{https://huggingface.co/docs/transformers/model_doc/bloom}} - 350m, 560m, 1b1, 1b3, 1b7, 2b5, 3b, and 7b1 that have significantly lesser storage and memory requirements. %Here m and b stand for the number of parameters in millions and billions, respectively, and the bold-faced variants have now been deprecated. %On the contrary, the two smallest variants 350m/560m and 1b3/1b7 require less than 5 GB of storage space and can be trained on 16 GB and 32 GB GPUs. 
%Thus, the work presented here focuses on evaluating the  smallest variants of the BLOOM model on various NLP tasks. 
%A benchmark of the performance of these variants can facilitate usage of the models i.. and how wwe e teaadvantage of this and benchmark the performance of these variants on several NLP tasks since they require much less computational resources.  
%This work presented in this paper evaluates the smaller BLOOM model variants on various Natural Language Processing (NLP) tasks to identify possible areas where the model(s) can be used. The experiments test the model syntactically as well as semantically in a traditional, Zero-shot and Few-shot manner. Additionally, the model variants are also evaluated using prompt-based text generation. The empirical results show that the model will bloom in a Few-shot setting, with the best performance observed on text extraction tasks in a Few-shot setting. An analysis of the model's failure to learn anything on a few tasks reveals how padding length impacts the learning process.
%The compute for training BLOOM was provided through a French public grant from GENCI and IDRIS, leveraging IDRIS’ Jean Zay supercomputer. The ROOTS corpus \cite{laurenon2022the} was used to train the BLOOM model. The corpus is a composite collection of 498 Hugging Face datasets \cite{lhoest-etal-2021-datasets}.
%We experiment and analyze the BLOOM model(s) on various NLP tasks. 

%for text extraction tasks, we observe an average 0.97\% increase in accuracy across all shots. Further, for text classification, for 2 out of 5 tasks, calibration of input results in the average accuracy across all shots increase by a minimum of 12.22\%. For the remaining three tasks, calibration actually decreases the accuracy of the model.
%The variants \textit{bloom} for prompt-based few-shot text extraction on MIT Movies and ATIS with $\sim$7\% greater accuracy over GPT-2 and GPT-Neo models on these datasets. (3) 

%We view the landscape of LLMs thorough the lens of the recently released BLOOM model. The BLOOM model is a generative LLM trained similar to GPT-2 but on large-scale multi-lingual data and with 176b parameters. We empirically observe that the model performance on a large variety of classification, generation, few shot and translation tasks does not scale with the size of the parameters [insert graph somewhere to support this claim, https://arxiv.org/pdf/2212.09803.pdf, https://arxiv.org/abs/2001.08361]. We also observe that BERT-style masked LMs are blah blah vs. Bloom and GPT. Moreover, even though Bloom was trained on 46 natural languages, its performance on MT on 6 languages the Amazon reviews dataset is comparable to GPT.

%ToDos-

%For point 1 of the abstract -
%- What is the difference in fine-tuning vs few-shot in terms of learning for BLOOM? Why is the same behaviour not seen in few-shot?

%-- Output variance based on prompt. GPT varies a lot.

%-- How reliably can leaderboard performance can be used to compare competing models -- from Parags BERTs vs. GPT/Bloom analysis on GLUE.
%100 sample analysis remains.

%For WNLI:
%BERT, GPT2, BLOOM-1b7, DeBERTa
%all predict 21 incorrectly
%all predict 33 correctly

\iffalse
-- How sensitive is the model to the order of inputs in case of few shot. experiments done -- analysis left. Bloom is generally less sensitive than GPT. Table accompanied by these observations.

Answer - The BLOOM model as compared to GPT2 and GPT3 models is not sensitive to the order of inputs. For text extraction tasks, an average increase in accuracy of 0.97 across all shots is seen. For text classification, for 2 out of 5 tasks, calibration of input results in the average accuracy across all shots increase by a minimum of 12.22\%. For the remaining three tasks, calibration actually decreases the accuracy of the model.

-- Toxicity of the generated texts - Using a model trained on toxic comment classification, we quantify the toxicity of the generated texts using gpt2, gpt3 and bloom-1b7 models. The dataset is taken from https://arxiv.org/abs/2009.11462. The scores show that text generated by gpt2 and gpt3 is more toxic as compared to bloom.  

Section on Why does Bloom underperform?
- Perf. does not scale with params
    - Analyze why does the larger model perform worse than the smaller variant
- Hyperparmeters and tuning?
- Underlying dataset?
- Does our qualitative error analysis on 100 samples support any of the above? Or any new observations from them.


Given leaderboards that help benchmark classification tasks (like GLUE/ SuperGLUE) and  sequence labeling (CoNLL NER), we characterize the performance of Bloom and other generative models vis-a-vis BERT-style masked language models. 

We also ran few-shot learning experiments similar to \cite{} on several popular classification tasks including sentiment analysis, entailment, question type classification and topic classification. In case of classification tasks GPT-2 mostly outperforms Bloom. 

In case of prompt based extraction tasks using MIT-Movies and ATIS, Bloom significantly? outperforms GPT-2 and GPT-Neo

Further, we test Bloom's a multi-lingual experiment, with the Amazon reviews corpus for 6 languages \cite{}. Performance here is simialr to GPT-2.

Bloom with 4-shot does 53.29\%. Bert using entire train does 60\%. RTE. 

Bloom doesnt follow scaling law. LLMs as size (params) increases, performance does not seem to improve.

- Why do GPT/other generative models outperform Bloom on GLUE?
Sample ~100 instances and analyze the following:
*WNLI? is Bloom able to generalize to the unseen instances in test? Bloom and DeBerta are comparable on this one -- some error analysis here? DeBErta was trained to do well on adversarial examples. In Bloom we do nothing -- maybe some points here.
* Take a task where Bloom does not do well but GPT and BERT do well -- error analysis. Also consider instances where BERT fails but GPT and Bloom do ok. Perhaps also where BERT and GPT fails, Bloom does better.
- How do BERT style models compare (qualitatively)  against Bloom/other generative models on GLUE?


%The experiments test the model syntactically as well as semantically in a traditional, Zero-shot and Few-shot manner. Additionally, the model variants are also evaluated using prompt-based text generation. The empirical results show that the model will bloom in a Few-shot setting, with the best performance observed on text extraction tasks in a Few-shot setting. An analysis of the model's failure to learn anything on a subset of tasks reveals how padding length impacts the learning process.


The 176B BLOOM model and its smaller variants were recently released as an open-source alternative to GPT-3. Although the model, training data and the training code are publicly available, the areas where models from the BLOOM family can be used are still unknown. Additionally, performance evaluation of the model primarily focuses on the 176B model variant, something that even for evaluation requires a large amount of compute. This work presented in this paper evaluates the smaller BLOOM model variants on various Natural Language Processing (NLP) tasks to identify possible areas where the model(s) can be used. The experiments test the model syntactically as well as semantically in a traditional, Zero-shot and Few-shot manner. Additionally, the model variants are also evaluated using prompt-based text generation. The empirical results show that the model will bloom in a Few-shot setting, with the best performance observed on text extraction tasks in a Few-shot setting. An analysis of the model's failure to learn anything on a few tasks reveals how padding length impacts the learning process.
\fi 

% \subsection{Practical considerations}

% Figure \ref{fig:runtime_comparison} compares all baselines evaluated on the GLUE tasks for the time taken to evaluate the QQP task post-fine-tuning (40k samples). The impact of the model's size is evident in the evaluation runtime, as shown in the figure.

% \begin{figure}[h]
%     \begin{center}
%         \includegraphics[width=0.45\textwidth]{runtime_comparison.png}
%     \end{center}
%     \caption{Comparison of the baselines with respect to evaluation time on the QQP validation set.}
%     \label{fig:runtime_comparison}
% \end{figure}

% \begin{figure}[h]
%     \begin{center}
%         \includegraphics[width=0.45\textwidth]{model_no_parameters.png}
%     \end{center}
%     \caption{Comparison of the baselines with respect to the number of parameters.}
%     \label{fig:model_parameter_comparison}
% \end{figure}

% In this section \ref{subsec:glue}, we highlight how the BLOOM model variants completely ignore one of the two classes in COLA predictions. This results in zero false and true negatives leading to a Matthews correlation score of 0.0. However, this is not the case with all other baselines evaluated for the GLUE tasks (see Table \ref{tab:glue_results}). We analyze this behavior further by experimenting with various training settings.

% \begin{enumerate}
%     \item Changing the class distribution in the training set: To force the model to learn predicting both the classes, we experiment with changing the class distribution to either balance it for both classes or favor the minority class (\textit{not entailment}) in varying degrees. These experiments resulted in the class predictions fluctuating between the two classes and changing the overall evaluation loss value start and resting value. They did not result in a positive non-zero Matthews correlation score.
%     \item Reducing the learning rate and increasing the number of epochs: The second hypothesis for the model's failure to predict both classes was a high learning rate resulting in oscillations between the classes. To test this hypothesis, we conduct multiple experiments with different learning rates - $2e-6$, $2e-8$, $2e-9$, and learning rate schedulers - linear and cosine. For all these experiments, we increase the number of epochs to 100. These experiments also do not result in increasing the Matthews correlation score above 0.0.
%     \item Gradient accumulation: Low batch sizes for the bloom variants can result in smaller weight updates. In order to ensure that this did not result in the model(s) ignoring one class, we do gradient accumulation to increase the number of batches resulting in a model weight update. We experiment with various values for the \textit{gradient\_accumulation\_steps} parameter - 8, 12, 16, 24, and 32. However, this also does not impact the Matthews correlation score.
%     \item Padding: Lastly, we analyze the output embeddings and input token ids of the model for various inputs and observe that majority of the tokens are \textit{PAD} tokens. In order to test the impact of padding, we experiment with different maximum values for the tokenized input - 16, 32, 64, 128, and 256. Setting the maximum sequence length to 128 resulted in a positive Matthews correlation score of 0.2 as the model was able to predict both classes for test inputs.
% \end{enumerate}

% \begin{table*}
%     \centering
%     \begin{tabular}{p{11em}cccccccccc}
%         \hline
%         \textbf{Dataset} & \textbf{Syn.} & \multicolumn{6}{c}{\textbf{Semantic}} & \textbf{Multi-} & \textbf{Zero-/} & \textbf{Tox.}\\
%         \cline{3-8}
%         & & \textbf{PD} & \textbf{TE} & \textbf{QA} & \textbf{SA} & \textbf{TU} & \textbf{EE} & \textbf{lingual} & \textbf{Few-shot} &\\
%         \hline
%         \hline
%         \textbf{GLUE} \cite{wang2019glue} & & & & & & & & & & \\
%         \cline{1-1}
%         \quad COLA \cite{warstadt-etal-2019-neural} & \checkmark & & & & & & & & & \\ 
%         \quad QNLI \cite{rajpurkar-etal-2016-squad} & &  & \checkmark & \checkmark & & & & & & \\
%         \quad MRPC \cite{dolan2005automatically} & & \checkmark & & & & & & & & \\
%         \quad STS-B  \cite{cer-etal-2017-semeval} & & \checkmark & & & & & & & & \\
%         \quad QQP\footnote{\url{https://data.quora.com/First-Quora-Dataset-Release-Question-Pairs}} & & \checkmark &  & & & & & & & \\
%         \quad SST2 \cite{socher2013recursive} & & & & & \checkmark & & & & \checkmark & \\
%         \quad RTE \cite{dagan2006pascal,bar2006second,giampiccolo-etal-2007-third,bentivogli2009fifth} & & & \checkmark & & & & & & \checkmark & \\
%         \quad WNLI \cite{levesque2011winograd} & & & \checkmark & & & & & & & \\
%         \quad MNLI \cite{bowman-etal-2015-large, williams-etal-2018-broad} & & & \checkmark & & & & & & & \\
%         \hline
%         \hline
%         SQuAD \cite{rajpurkar-etal-2016-squad} & & & & \checkmark & & & & & & \\
%         \hline
%         \hline
%         AGNews \cite{zhang2015character} & & & & & & \checkmark & & & \checkmark & \\
%         TREC \cite{voorhees2000building} & & & & \checkmark & & & & & \checkmark & \\
%         CB \cite{de2019commitmentbank} & & & \checkmark & & & & & & \checkmark & \\
%         ATIS \cite{hemphill-etal-1990-atis} & & & & & & & \checkmark & & \checkmark & \\
%         MIT Movies \cite{liu2012conversational} & & & & & & & \checkmark & & \checkmark & \\
%         \hline
%         \hline
%         XNLI \cite{conneau-etal-2018-xnli} & & & \checkmark & & & & & \checkmark & & \\
%         MARC \cite{marc_reviews} & & & & & & & & \checkmark & & \\
%         \hline
%         \hline
%         ParaQA \cite{kacupaj2021paraqa} & & & & \checkmark & & & & & & \\
%         FiQA \cite{10.1145/3184558.3192301} & & & & \checkmark & & & & & & \\
%         NewsData\footnote{\url{https://www.kaggle.com/datasets/gennadiyr/us-equities-news-data}} & & & & & & \checkmark & & & & \\
%         \hline
%         \hline
%         CoNLL++ \cite{wang-etal-2019-crossweigh} & & & & & & \checkmark & & & & \\
%         \hline
%         \hline
%         RealToxicityPrompts \cite{gehman-etal-2020-realtoxicityprompts} & & & & & & & & & & \checkmark\\
%         \hline
%     \end{tabular}
%     \caption{\label{tab:few-shot-text-extraction} Results of few-shot learning experiments all the baselines on text-extraction tasks.}
% \end{table*}

% \begin{table*}
%     \centering
%     \begin{tabular}{lp{2em}p{3em}p{3em}p{3em}p{3em}p{3em}p{3em}p{3em}}
%         \hline
%         \textbf{Models} & \textbf{Shot} & \textbf{replaced with} & \textbf{refers to} & \textbf{represent} & \textbf{the pronoun p refers to} & \textbf{What does p stand for} & \textbf{by p they mean} & \textbf{who or what is/are}\\
%         \hline
%         gpt2-xl & 0 & & & & & & &\\
%         & 1 & 37.07$_{2.69}$ & 42.58$_{3.44}$ & 45.51$_{1.97}$ & 33.99$_{3.46}$ & 35.86$_{1.80}$ & 39.49$_{3.37}$ & 27.78$_{8.94}$\\
%         \cline{2-9}
%         gpt-neo & 0 & 0.0 & 0.0 & 0.0 & 0.25 & 0.0 & 0.25 & 0.25\\
%         & 1 & 38.69$_{5.78}$ & 44.80$_{5.64}$ & 44.49$_{4.67}$ & 31.62$_{9.36}$ & 25.20$_{8.41}$ & 34.29$_{7.13}$ & 12.83$_{6.50}$\\
%         \cline{2-9}
%         bloom-1b7 & 0 & & & & & & &\\
%         & 1 & 38.69$_{5.78}$ & 44.80$_{5.64}$ & 44.49$_{4.67}$ & 31.62$_{9.36}$ & 25.20$_{8.41}$ & 34.29$_{7.13}$ & 12.83$_{6.50}$\\
%         \hline
%     \end{tabular}
%     \caption{\label{tab:conll_task_scores} Results of Zero-/One-shot learning on the WinoBias dataset}
% \end{table*}

% \begin{table*}
%     \centering
%     \begin{tabular}{lp{2em}p{3em}p{3em}p{3em}p{3em}p{3em}p{3em}p{3em}}
%         \hline
%         \textbf{Models} & \textbf{Shot} & \textbf{replaced with} & \textbf{refers to} & \textbf{represent} & \textbf{the pronoun p refers to} & \textbf{What does p stand for} & \textbf{by p they mean} & \textbf{who or what is/are}\\
%         \hline
%         gpt2-medium & 0 & 0.0$_{0.0}$ & 0.0$_{0.0}$ & 0.0$_{0.0}$ & 0.0$_{0.0}$ & 0.0$_{0.0}$ & 0.25$_{0.0}$ & 0.0$_{0.0}$\\
%         & 1 & 38.69$_{5.78}$ & 44.80$_{5.64}$ & 44.49$_{4.67}$ & 31.62$_{9.36}$ & 25.20$_{8.41}$ & 34.29$_{7.13}$ & 12.83$_{6.50}$\\
%         \cline{2-9}
%         gpt2-xl & 0 & & & & & & &\\
%         & 1 & 37.07$_{2.69}$ & 42.58$_{3.44}$ & 45.51$_{1.97}$ & 33.99$_{3.46}$ & 35.86$_{1.80}$ & 39.49$_{3.37}$ & 27.78$_{8.94}$\\
%         \cline{2-9}
%         gpt-neo & 0 & & & & & & &\\
%         & 1 & 38.69$_{5.78}$ & 44.80$_{5.64}$ & 44.49$_{4.67}$ & 31.62$_{9.36}$ & 25.20$_{8.41}$ & 34.29$_{7.13}$ & 12.83$_{6.50}$\\
%         \cline{2-9}
%         bloom-560m & 0 & 0.0$_{0.0}$ & 0.0$_{0.0}$ & 0.0$_{0.0}$ & 0.0$_{0.0}$ & 0.0$_{0.0}$ & 0.25$_{0.0}$ & 0.0$_{0.0}$\\
%         & 1 & 38.69$_{5.78}$ & 44.80$_{5.64}$ & 44.49$_{4.67}$ & 31.62$_{9.36}$ & 25.20$_{8.41}$ & 34.29$_{7.13}$ & 12.83$_{6.50}$\\
%         \cline{2-9}
%         bloom-1b7 & 0 & & & & & & &\\
%         & 1 & 38.69$_{5.78}$ & 44.80$_{5.64}$ & 44.49$_{4.67}$ & 31.62$_{9.36}$ & 25.20$_{8.41}$ & 34.29$_{7.13}$ & 12.83$_{6.50}$\\
%         \hline
%     \end{tabular}
%     \caption{\label{tab:conll_task_scores} Results of Zero-/One-shot learning on the WinoBias dataset}
% \end{table*}

% \begin{enumerate}
%     \itemsep0em
%     \item Question classification to understand how well a model can identify question types
%     \item Answer detection to test if the model can detect if a given sentence contains an answer to a given question
%     \item Question answering to see if a model can answer a question from a given context
%     \item Answer generation to evaluate a model's answer generation capability and if it can remember facts seen during training.
% \end{enumerate}
